Enabling Hard Constraints in Differentiable Neural Network and Accelerator Co-Exploration

Co-exploration of an optimal neural architecture and its hardware accelerator is an approach of rising interest which addresses the computational cost problem, especially in low-profile systems. The large co-exploration space is often handled by adopting the idea of differentiable neural architecture search. However, despite the superior search efficiency of the differentiable co-exploration, it faces a critical challenge of not being able to systematically satisfy hard constraints such as frame rate. To handle the hard constraint problem of differentiable co-exploration, we propose HDX, which searches for hard-constrained solutions without compromising the global design objectives. By manipulating the gradients in the interest of the given hard constraint, high-quality solutions satisfying the constraint can be obtained.

==> discussion.tex <==

\vspace{-1mm}
\section{Discussion}
\vspace{-1mm}

%\KH{Did finger snap, please check} 
\textbf{One-shot NAS methods.} 
Recently, one-shot NAS methods \citep{ofa,one-shot,nayman2021hardcorenas} are drawing much attention, 
% By sharing kernel weights among multiple kernel sizes and channel width, 
which trains the supernet only once and searches for a sub-network for a given purpose.
% or auxiliary training. 
% Therefore, one might say that one-shot NAS methods are applicable for a constrained co-search problem with na\"ive exhaustive search. 
%Even though one-shot NAS methods eliminate the need for repetitive training of sampled networks, 
However, one-shot NAS method is not a directly satisfying solution for the constrained co-search task.
First, 
%they still require gigantic search cost for the constrained co-search problem. 
%For instance, Once-For-All \citep{ofa} has total ${2\times10^{19}}$ networks in the search space\KH{need example?}. 
%Putting network performance evaluation costs aside, 
hardware metrics of each network need to be measured on the whole hardware accelerator search space, then compared with each other, which is a non-trivial process that takes a long time. %and compared  
% Specifically, to rank which hardware accelerator is better and to examine the accelerator-network pair  meet the resource constraint still require considerable computational cost. 
Furthermore, cost for training the entire supernet itself is often multiple times more expensive than that of a conventional differentiable NAS, and searching for each subnetwork is also costly, making the break-even number of deployments very high.


% As one-shot NAS method is considered a sub-category of many differentiable NAS methods, 
Nonetheless, if multiple deployments are planned over diverse constraints, we believe \methodname can utilize one-shot NAS as its backbone thanks to its differentiability. 
One way to apply one-shot NAS method onto \methodname is to attach differentiable architecture selector on pre-trained supernet. 
%The architecture selector is jointly trained with hardware generator to co-explore neural network and hardware architecture search space.
Since both components are differentiable neural networks, gradient manipulation technique can be applied to them in a coherent manner.
% One-shot NAS backbone not only reduces computation resource on exploring network search space but improves network performance thanks to the strength of the one-shot NAS backbone itself. 
Expanding our experiment further to include one-shot NAS as our network search backbone is left as future work. 
% We are planning to include a one-shot NAS method in the network search backbone of our method as future work.

\textbf{Expanding Design Space.} One might wonder whether the scheme used in \methodname can be applied to other co-exploration methods. 
For example, \citet{li2020edd} and \citet{fu2021autonba} optimize the quantization level of each layer in addition to the neural architecture.
We believe \methodname can accommodate such additional design space into consideration.
Provided that there exists a analytic or simulation model for those additional spaces (which is not difficult to build),
satisfying hard-constraint through gradient manipulation is likely to work with little extra effort.
%Even though using the exact same exploration methods from \citep{li2020edd,fu2021autonba} might not directly work due to the way they express the hardware-network relation, 

==> iclr2022/discussion.tex <==

\vspace{-1mm}
\section{Discussion}
\vspace{-1mm}

%\KH{Did finger snap, please check} 
\textbf{One-shot NAS methods.} 
Recently, one-shot NAS methods \citep{ofa,one-shot,nayman2021hardcorenas} are drawing much attention, 
% By sharing kernel weights among multiple kernel sizes and channel width, 
which trains the supernet only once and searches for a sub-network for a given purpose.
% or auxiliary training. 
% Therefore, one might say that one-shot NAS methods are applicable for a constrained co-search problem with na\"ive exhaustive search. 
%Even though one-shot NAS methods eliminate the need for repetitive training of sampled networks, 
However, one-shot NAS method is not a directly satisfying solution for the constrained co-search task.
First, 
%they still require gigantic search cost for the constrained co-search problem. 
%For instance, Once-For-All \citep{ofa} has total ${2\times10^{19}}$ networks in the search space\KH{need example?}. 
%Putting network performance evaluation costs aside, 
hardware metrics of each network need to be measured on the whole hardware accelerator search space, then compared with each other, which is a non-trivial process that takes a long time. %and compared  
% Specifically, to rank which hardware accelerator is better and to examine the accelerator-network pair  meet the resource constraint still require considerable computational cost. 
Furthermore, cost for training the entire supernet itself is often multiple times more expensive than that of a conventional differentiable NAS, and searching for each subnetwork is also costly, making the break-even number of deployments very high.


% As one-shot NAS method is considered a sub-category of many differentiable NAS methods, 
Nonetheless, if multiple deployments are planned over diverse constraints, we believe \methodname can utilize one-shot NAS as its backbone thanks to its differentiability. 
One way to apply one-shot NAS method onto \methodname is to attach differentiable architecture selector on pre-trained supernet. 
%The architecture selector is jointly trained with hardware generator to co-explore neural network and hardware architecture search space.
Since both components are differentiable neural networks, gradient manipulation technique can be applied to them in a coherent manner.
% One-shot NAS backbone not only reduces computation resource on exploring network search space but improves network performance thanks to the strength of the one-shot NAS backbone itself. 
Expanding our experiment further to include one-shot NAS as our network search backbone is left as future work. 
% We are planning to include a one-shot NAS method in the network search backbone of our method as future work.

\textbf{Expanding Design Space.} One might wonder whether the scheme used in \methodname can be applied to other co-exploration methods. 
For example, \citet{li2020edd} and \citet{fu2021autonba} optimize the quantization level of each layer in addition to the neural architecture.
We believe \methodname can accommodate such additional design space into consideration.
Provided that there exists a analytic or simulation model for those additional spaces (which is not difficult to build),
satisfying hard-constraint through gradient manipulation is likely to work with little extra effort.
%Even though using the exact same exploration methods from \citep{li2020edd,fu2021autonba} might not directly work due to the way they express the hardware-network relation, 

==> iclr2022/figs/table_quality.tex <==

\begin{table}[b]
\setlength{\tabcolsep}{2pt}
\vspace{-3mm}
    \centering
    \footnotesize
    \caption{Results Showing the Quality of Solutions \vspace{-3mm}}
    \label{tab:quality}
    \begin{tabular}{clcccccc}
    \toprule
         Index & Constrained & Lat. (\SI{}{\milli\second}) & E (\SI{}{\milli\joule}) & Area ($\SI{}{\milli\meter\squared}$)  & Error (\%) & $Cost_{HW}$ &  Loss \\
\midrule
\multirow{5}{*}{A}  & Anchor  & \textcolor{blue}{69.23} & \textcolor{olivegreen}{37.00} & \textcolor{orange}{2.53} & 4.10 $\pm$ 0.16 & 21.84 & 0.632 \\%&1&latency_0001_no_const
\cmidrule(lr){2-8}
                    & Latency           & \textbf{\textcolor{blue}{43.99}} & 21.79 & 2.10 & 4.20 $\pm$ 0.07 & 13.87 & 0.624 \\%&21&const_1_of_const_3_latency_0001_latency_19
                    & Energy            & 51.98 & \textbf{\textcolor{olivegreen}{29.18}} & 2.53 & 4.38 $\pm$ 0.17 & 17.44 & 0.630 \\%&22&const_1_of_const_3_latency_0001_energy_18
                    & Chip Area         & 64.00 & 34.82 & \textbf{\textcolor{orange}{2.53}} & 4.05 $\pm$ 0.06 & 20.56 & 0.629 \\%&23&const_1_of_const_3_latency_0001_area_20
                    & All               & \textbf{\textcolor{blue}{63.72}} & \textbf{\textcolor{olivegreen}{12.09}} & \textbf{\textcolor{orange}{1.86}} & 4.12 $\pm$ 0.18 & 13.29 & 0.623 \\%&2&3const_latency_0001
\midrule%&%&&&&&&&\\%&&
\multirow{5}{*}{B}  & Anchor  & \textcolor{blue}{49.65} & \textcolor{olivegreen}{27.53} & \textcolor{orange}{2.53} & 4.22 $\pm$ 0.06 & 16.67 & 0.638 \\%&3&latency_0002_no_const
\cmidrule(lr){2-8}
                    & Latency           & \textbf{\textcolor{blue}{48.02}} & 27.33 & 2.53 & 4.27 $\pm$ 0.09 & 16.41 & 0.644 \\%&24&const_1_of_const_3_latency_0002_latency_15
                    & Energy            & 95.02 & \textbf{\textcolor{olivegreen}{24.45}} & 1.89 & 4.05 $\pm$ 0.10 & 20.76 & 0.648 \\%&25&const_1_of_const_3_latency_0002_energy_14
                    & Chip Area         & 54.74 & 29.81 & \textbf{\textcolor{orange}{2.53}} & 4.11 $\pm$ 0.13 & 17.96 & 0.645 \\%&26&const_1_of_const_3_latency_0002_area_20
                    & All               & \textbf{\textcolor{blue}{41.32}} &  {\color{white}0}\textbf{\textcolor{olivegreen}{8.59}} & \textbf{\textcolor{orange}{1.86}} & 4.35 $\pm$ 0.05 &  {\color{white}0}9.50 & 0.629 \\%&4&3const_latency_0002
%\midrule%&%&&&&&&\\%&&
% \multirow{5}{*}{C}  & Anchor & \textcolor{blue}{56.11} & \textcolor{olivegreen}{29.81} & \textcolor{orange}{2.53} & 4.11 $\pm$ 0.10 & 18.13 & 0.662 \\%&5&latency_0003_no_const
%                     & Latency           & \textbf{\textcolor{blue}{51.81}} &  {\color{white}0}9.49 & 1.89 & 4.38 $\pm$ 0.11 & 11.06 & 0.645 \\%&27&const_1_of_const_3_latency_0003_latency_15
%                     & Energy            & 44.78 & \textbf{\textcolor{olivegreen}{24.38}} & 2.53 & 4.12 $\pm$ 0.02 & 15.15 & 0.656 \\%&28&const_1_of_const_3_latency_0003_energy_13
%                     & Chip Area         & 53.37 & 26.63 & \textbf{\textcolor{orange}{2.10}} & 4.43 $\pm$ 0.07 & 16.44 & 0.668 \\%&29&const_1_of_const_3_latency_0003_area_19
%                     & All               & \textbf{\textcolor{blue}{41.53}} &  {\color{white}0}\textbf{\textcolor{olivegreen}{8.81}} & \textbf{\textcolor{orange}{1.86}} & 4.48 $\pm$ 0.20 & {\color{white}0}9.59 & 0.645 \\%&6&3const_latency_0003

        \bottomrule
        \multicolumn{8}{r}{*Bold colored numbers indicate that they are}  \\
        \multicolumn{8}{r}{under constraint of the same colored non-bold numbers.}
        \vspace{-3mm}
    \end{tabular}
\end{table}

==> iclr2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2022/oldintro.tex <==
% have emerged ->?
Since the main interest of most \emph{Deep Neural Network} (DNN) researches has always been accuracy, models have grown larger to achieve the goal and it induces excessive compute intensities.
% Ever since \emph{Deep Neural Network} (DNN) researches have emerged, the main interest of most researchers has always been the accuracy of models.
% To achieve this goal, models have grown larger and it induces excessive compute intensities.
This has put burden on people with limiting computing power, making it difficult to benefit from SoTA DNNs.\HY{I feel like this paragraph can be summed up in a sentence} \DK{decentralization?}
In recent years, many works have appeared to deal with this problem and most of them belong to one of these two ways - \emph{network-side optimization} and \emph{hardware-side optimization}.
% This issue is usually dealt in two ways - \emph{network-side optimization} and \emph{hardware-side optimization}.
% In order to use DNNs in practice while avoiding the above issue, there are several conditions to be satisfied - \emph{lightweight network}, \emph{optimized hardware}, \emph{constraints to be met}.
% In recent years, many works have appeared in the field of optimizing DNNs in terms of both accuracy and efficiency and most of their approaches usually belong to one of them.
% most of their approaches can be categorized as meeting one of these conditions.
% lightweight network -> ?
\emph{Network-side optimization} refers to refining the architecture of a network or optimizing operations within a network to reduce computations while maintaining comparable accuracy as large networks. %For example, depth-wise separable convolution operation \cite{mobilenet} achieves low latency due to its reduced computational cost while maintaining high accuracy. \HY{The whole example seems redundant and unnecessary. Maybe elaborate more on the definition itself?}
\emph{Hardware-size optimization}, on the other hand, refers to improving DNN execution efficiency by using an optimized hardware design, also known as an \emph{Accelerator}.
% Numerous works execute DNNs on their own hardwares to attain low latency and/or low energy consumption.
% For instance, a renowned accelerator, Google's TPU\cite{tpu} is used to accelerate the processing of AlphaGo \cite{alphagozero}. \HY{same here}
Other existing works devise frameworks to evaluate DNN accelerator's latency (\cite{timeloop}) or energy (\cite{accelergy}), and they can be employed to find better accelerators for given network. 

% \emph{Constraints to be met} is related to practically inevitable limitations in order to use DNN in real life.
% There are some tasks that should guarantee a certain level of hardware metrics.
% For example, autonomous driving has to promise low latency to cope with any possible situations on the road \cite{e2eauto}.
% Also, there can be some limitations about energy consumption or chip size when a neural network is executed on an edge device.
% No matter how high the accuracy of given network is, even though an optimal hardware accelerator architecture of given network is already found, they can't be used if they don't meet given constraint(s).

Although these methods are essential for DNN applications, it is hard to satisfy them at the same time.
% First of all,\HY{rm First of all?}
Suppose there is a need an efficient neural network and hardware accelerator pair.
Considering network-side effort and hardware-side effort only, it will be best if both methods are applied simultaneously and take advantages from each of them.
Unfortunately, Although the purpose of both methods is the same, but one effort hinders another effort.
% they don't work out as expected.
%The purpose\HY{I don't think this should be plural} of both methods is the same, but one effort hinders another effort.
For example, the main advantage of depth-wise separable convolution operation\cite{mobilenet} is from its structure that its intermediate channel is 1.
Therefore it can't be parallelized well with TPU\cite{tpu}, a renowned accelerator, because the main advantage of it is channel-wise parallelism \cite{edgetpunas}.

That's why neural network architecture and accelerator architecture should be considered at the same time.\textcolor{purple}{DK:[that's why....]}
\emph{Neural Architecture Search} (NAS) has emerged as an efficient way to address this co-optimization problem. \HY{I feel like the paragraph should begin with this sentence}
% \emph{Neural Architecture Search} (NAS) is another way to optimize accuracy and efficiency simultaneously.
% NAS is an automated technique for design neural network architecture.
NAS started off as a method to find networks which achieve good accuracy without human effort \cite{mnasnet, darts}.
Nowadays, researchers consider to optimize hardware related metrics such as latency or energy with NAS \cite{proxylessnas}.
% \textcolor{purple}{DK:[too short]}
Most of the existing methods are based on Reinforcement Learning \cite{cosearch, cosearch_fpga, cosearch_fpga2, cosearch_multi, cosearch_bestofboth}.
They first sample a neural network from network search space and find optimal hardware accelerator of the network.
After train the network, update reward function with accuracy of the network and hardware metrics from the network and the optimal hardware accelerator which is already found.
This method is good to find optimal solution.
But to get a solution, hundreds of thousands of networks should be trained and should find optimal accelerator architecture of each of them for updating reward function.
That is, the cost of RL based method is too heavy.
Also, if search is stopped because of that enormous costs, the solution can be suboptimal.
Another way to explore both search space concurrently is searching both space differentiably.
Differentiable NAS is a way to find optimal network without RL by training super network and sampling a sub network from super network.
Super network has many operations in each layer and they are connected densely.
While training, not only weights of each operation are updated, but also architecture parameters which denote path of sub network are updated, too.
With this in mind, optimal hardware accelerator architecture also can be searched differentiably.
First work which implements this method \cite{edd} tries to formulate a relation of neural network and accelerator architecture, but that formulation can't truly reflect their relation.
A paper called \emph{DANCE} \cite{dance} solves this problem by training a network which finds optimal accelerator architecture of given network and approximates hardware metrics of the network-accelerator pair at the same time.
By adding a loss term of hardware metrics which from the pre-trained network called \emph{Evaluator}, it optimizes network architecture and accelerator architecture by propagating gradients for hardware metrics to super network via Evaluator.

Giving constraints about hardware metrics has a similar problem.
There are already some works to find networks which comply with given constraints.
This problem also can solve by using RL \cite{rcnas_edge}.
But because it is a kind of RL based NAS, its cost is huge.
One of other ways is shrinking search space gradually.
It can be done by fixing most optimal operation step by step \cite{rcnet} or removing worst operation from search space \cite{hardcorenas}.
Unfortunately, what these methods have in common is they assume that hardware accelerator structure which will execute DNN is fixed.
It means that there can be better solutions by refining their accelerator architecture.
That is, these methods are appropriate to solve constrained NAS, but it doesn't fit well to co-search problem because approximations for optimization can be changed while optimal accelerator architecture has changed.

To sum up, it is hard to co-search optimal network and accelerator pair which conform to given constraints.
It can be solved with RL, but it is too costly.
With differentiable co-search method, it may not be able to reach solution space under constraints.
Differentiable and constrained NAS also has a problem, which is valid solution spaces keep changing as intermediate optimal network or accelerator architecture changed. 
Therefore there need a novel method to conduct co-search while satisfying all of three conditions in reasonable time.

In order to solve this problem, we present \emph{CoDE} (Constrained Differentiable Explorer for network/accelerator), which can reduce search cost of network architecture and accelerator architecture while gives constraints to hardware metrics.
This work uses pre-trained network for get approximated hardware metrics for current optimal network and accelerator like DANCE.
% instead of shrinking search space, 
But, while searching, it can prevent searched network and accelerator from violating given constraints by manipulating gradients to comply with constraints \cite{dpm}.
By doing this, it can co-explore both search spaces pulling each of them into the valid solution space when searched network-accelerator pair don't abide by given constraints.
Also, CoDE can do this with reasonable amount of time without shrinking search spaces.
To the best of our knowledge, this is first paper that co-search neural network architecture and hardware accelerator architecture at the same time while giving constraints to hardware metrics.

Our contributions are as follows.
\begin{itemize}
    \item We propose a differentiable and constrained co-search method for network and accelerator architectures in order to find valid solutions when some resources are limited.
    \item We provide an efficient exploration method which traverses valid solution spaces under constraints.
\end{itemize}

==> iclr2022/packages.tex <==


% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\input{math_commands.tex}

\usepackage{hyperref}
\usepackage{url}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{subcaption}
\usepackage{verbatim} % begin comment
\usepackage{booktabs} % toprule, midrule, bottomrule

\usepackage{multirow}
\usepackage{array, makecell} %
\usepackage{siunitx}
\usepackage{alphalph} %for auto title \alph
\usepackage{tablefootnote}


\usepackage{enumitem}


%\usepackage[numbers,maxbibnames=2]{natbib}

\usepackage[export]{adjustbox} % for left, right in includegraphics

%taken from CVPR 2022
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Table}{Tables}
%\crefname{table}{Tab.}{Tabs.}


\definecolor{olivegreen}{rgb}{0, 0.6, 0}
\newcommand{\JL}[1]{{\color{olivegreen}[\textbf{\sc JLee}: \textit{#1}]}}
\newcommand{\rev}[1]{{\color{blue}[#1]}}
\newcommand{\KH}[1]{{\color{purple}[\textbf{\sc KH}: \textit{#1}]}}
\newcommand{\HY}[1]{{\color{blue}[\textbf{\sc HY}: \textit{#1}]}}
\newcommand{\DK}[1]{{\color{teal}[\textbf{\sc DK}: \textit{#1}]}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\renewcommand{\JL}[1]{}
%\renewcommand{\rev}[1]{}
\renewcommand{\KH}[1]{}
\renewcommand{\HY}[1]{}
\renewcommand{\DK}[1]{}
\renewcommand{\fix}{}
\renewcommand{\new}{}


\newcommand{\methodname}{HDX\xspace}



\newcommand{\eq}[1]{Eq.~\ref{eq:#1}\xspace}


\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{groupplots}
\usepackage{tikz}
\usetikzlibrary{patterns}



\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\color{olivegreen}\ding{51}}%
\newcommand{\xmark}{\color{red}\ding{55}}%

==> oldintro.tex <==
% have emerged ->?
Since the main interest of most \emph{Deep Neural Network} (DNN) researches has always been accuracy, models have grown larger to achieve the goal and it induces excessive compute intensities.
% Ever since \emph{Deep Neural Network} (DNN) researches have emerged, the main interest of most researchers has always been the accuracy of models.
% To achieve this goal, models have grown larger and it induces excessive compute intensities.
This has put burden on people with limiting computing power, making it difficult to benefit from SoTA DNNs.\HY{I feel like this paragraph can be summed up in a sentence} \DK{decentralization?}
In recent years, many works have appeared to deal with this problem and most of them belong to one of these two ways - \emph{network-side optimization} and \emph{hardware-side optimization}.
% This issue is usually dealt in two ways - \emph{network-side optimization} and \emph{hardware-side optimization}.
% In order to use DNNs in practice while avoiding the above issue, there are several conditions to be satisfied - \emph{lightweight network}, \emph{optimized hardware}, \emph{constraints to be met}.
% In recent years, many works have appeared in the field of optimizing DNNs in terms of both accuracy and efficiency and most of their approaches usually belong to one of them.
% most of their approaches can be categorized as meeting one of these conditions.
% lightweight network -> ?
\emph{Network-side optimization} refers to refining the architecture of a network or optimizing operations within a network to reduce computations while maintaining comparable accuracy as large networks. %For example, depth-wise separable convolution operation \cite{mobilenet} achieves low latency due to its reduced computational cost while maintaining high accuracy. \HY{The whole example seems redundant and unnecessary. Maybe elaborate more on the definition itself?}
\emph{Hardware-size optimization}, on the other hand, refers to improving DNN execution efficiency by using an optimized hardware design, also known as an \emph{Accelerator}.
% Numerous works execute DNNs on their own hardwares to attain low latency and/or low energy consumption.
% For instance, a renowned accelerator, Google's TPU\cite{tpu} is used to accelerate the processing of AlphaGo \cite{alphagozero}. \HY{same here}
Other existing works devise frameworks to evaluate DNN accelerator's latency (\cite{timeloop}) or energy (\cite{accelergy}), and they can be employed to find better accelerators for given network. 

% \emph{Constraints to be met} is related to practically inevitable limitations in order to use DNN in real life.
% There are some tasks that should guarantee a certain level of hardware metrics.
% For example, autonomous driving has to promise low latency to cope with any possible situations on the road \cite{e2eauto}.
% Also, there can be some limitations about energy consumption or chip size when a neural network is executed on an edge device.
% No matter how high the accuracy of given network is, even though an optimal hardware accelerator architecture of given network is already found, they can't be used if they don't meet given constraint(s).

Although these methods are essential for DNN applications, it is hard to satisfy them at the same time.
% First of all,\HY{rm First of all?}
Suppose there is a need an efficient neural network and hardware accelerator pair.
Considering network-side effort and hardware-side effort only, it will be best if both methods are applied simultaneously and take advantages from each of them.
Unfortunately, Although the purpose of both methods is the same, but one effort hinders another effort.
% they don't work out as expected.
%The purpose\HY{I don't think this should be plural} of both methods is the same, but one effort hinders another effort.
For example, the main advantage of depth-wise separable convolution operation\cite{mobilenet} is from its structure that its intermediate channel is 1.
Therefore it can't be parallelized well with TPU\cite{tpu}, a renowned accelerator, because the main advantage of it is channel-wise parallelism \cite{edgetpunas}.

That's why neural network architecture and accelerator architecture should be considered at the same time.\textcolor{purple}{DK:[that's why....]}
\emph{Neural Architecture Search} (NAS) has emerged as an efficient way to address this co-optimization problem. \HY{I feel like the paragraph should begin with this sentence}
% \emph{Neural Architecture Search} (NAS) is another way to optimize accuracy and efficiency simultaneously.
% NAS is an automated technique for design neural network architecture.
NAS started off as a method to find networks which achieve good accuracy without human effort \cite{mnasnet, darts}.
Nowadays, researchers consider to optimize hardware related metrics such as latency or energy with NAS \cite{proxylessnas}.
% \textcolor{purple}{DK:[too short]}
Most of the existing methods are based on Reinforcement Learning \cite{cosearch, cosearch_fpga, cosearch_fpga2, cosearch_multi, cosearch_bestofboth}.
They first sample a neural network from network search space and find optimal hardware accelerator of the network.
After train the network, update reward function with accuracy of the network and hardware metrics from the network and the optimal hardware accelerator which is already found.
This method is good to find optimal solution.
But to get a solution, hundreds of thousands of networks should be trained and should find optimal accelerator architecture of each of them for updating reward function.
That is, the cost of RL based method is too heavy.
Also, if search is stopped because of that enormous costs, the solution can be suboptimal.
Another way to explore both search space concurrently is searching both space differentiably.
Differentiable NAS is a way to find optimal network without RL by training super network and sampling a sub network from super network.
Super network has many operations in each layer and they are connected densely.
While training, not only weights of each operation are updated, but also architecture parameters which denote path of sub network are updated, too.
With this in mind, optimal hardware accelerator architecture also can be searched differentiably.
First work which implements this method \cite{edd} tries to formulate a relation of neural network and accelerator architecture, but that formulation can't truly reflect their relation.
A paper called \emph{DANCE} \cite{dance} solves this problem by training a network which finds optimal accelerator architecture of given network and approximates hardware metrics of the network-accelerator pair at the same time.
By adding a loss term of hardware metrics which from the pre-trained network called \emph{Evaluator}, it optimizes network architecture and accelerator architecture by propagating gradients for hardware metrics to super network via Evaluator.

Giving constraints about hardware metrics has a similar problem.
There are already some works to find networks which comply with given constraints.
This problem also can solve by using RL \cite{rcnas_edge}.
But because it is a kind of RL based NAS, its cost is huge.
One of other ways is shrinking search space gradually.
It can be done by fixing most optimal operation step by step \cite{rcnet} or removing worst operation from search space \cite{hardcorenas}.
Unfortunately, what these methods have in common is they assume that hardware accelerator structure which will execute DNN is fixed.
It means that there can be better solutions by refining their accelerator architecture.
That is, these methods are appropriate to solve constrained NAS, but it doesn't fit well to co-search problem because approximations for optimization can be changed while optimal accelerator architecture has changed.

To sum up, it is hard to co-search optimal network and accelerator pair which conform to given constraints.
It can be solved with RL, but it is too costly.
With differentiable co-search method, it may not be able to reach solution space under constraints.
Differentiable and constrained NAS also has a problem, which is valid solution spaces keep changing as intermediate optimal network or accelerator architecture changed. 
Therefore there need a novel method to conduct co-search while satisfying all of three conditions in reasonable time.

In order to solve this problem, we present \emph{CoDE} (Constrained Differentiable Explorer for network/accelerator), which can reduce search cost of network architecture and accelerator architecture while gives constraints to hardware metrics.
This work uses pre-trained network for get approximated hardware metrics for current optimal network and accelerator like DANCE.
% instead of shrinking search space, 
But, while searching, it can prevent searched network and accelerator from violating given constraints by manipulating gradients to comply with constraints \cite{dpm}.
By doing this, it can co-explore both search spaces pulling each of them into the valid solution space when searched network-accelerator pair don't abide by given constraints.
Also, CoDE can do this with reasonable amount of time without shrinking search spaces.
To the best of our knowledge, this is first paper that co-search neural network architecture and hardware accelerator architecture at the same time while giving constraints to hardware metrics.

Our contributions are as follows.
\begin{itemize}
    \item We propose a differentiable and constrained co-search method for network and accelerator architectures in order to find valid solutions when some resources are limited.
    \item We provide an efficient exploration method which traverses valid solution spaces under constraints.
\end{itemize}
